NetNN: Neural Intrusion Detection System in Programmable Networks

The rise of deep learning has led to various successful attempts to apply deep neural networks (DNNs) for important networking tasks such as intrusion detection. Yet, running DNNs in the network control plane, as typically done in existing proposals, suffers from high latency that impedes the practicality of such approaches. This paper introduces NetNN, a novel DNN-based intrusion detection system that runs completely in the network data plane to achieve low latency. NetNN adopts raw packet information as input, avoiding complicated feature engineering. NetNN mimics the DNN dataflow execution by mapping DNN parts to a network of programmable switches, executing partial DNN computations on individual switches, and generating packets carrying intermediate execution results between these switches. We implement NetNN in P4 and demonstrate the feasibility of such an approach. Experimental results show that NetNN can improve the intrusion detection accuracy to 99\% while meeting the real-time requirement.

==> sections/04-implementation.tex <==
\section{Implementation} \label{sec:implementation}


==> sections/10-extra.tex <==
\section{Extra}

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.45\textwidth]{figures/concatenated_bits_512_500.png}
    % \vspace{-0.1cm}
    
    \caption{Concatenated, validation accuracy: 55\%} \label{fig:conc}
    % \vspace{-0.4cm}
\end{figure}

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.45\textwidth]{figures/concatenated_bits_extra_512_500.png}
    % \vspace{-0.1cm}
    
    \caption{Concatenated with flow feature of the chosen packets, validation accuracy: 49\%} \label{fig:conc_extra}
    % \vspace{-0.4cm}
\end{figure}

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.45\textwidth]{figures/concatenated_bits_extra_all_512_1500.png}
    % \vspace{-0.1cm}
    
    \caption{Concatenated with flow features of all packets, validation accuracy: 58\%} \label{fig:conc_all}
    % \vspace{-0.4cm}
\end{figure}

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.45\textwidth]{figures/separated_1024_1000_10.png}
    \caption{Separated, validation split=10\%, validation accuracy: 96\%} \label{fig:sep}
    % \vspace{-0.4cm}
\end{figure}

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.45\textwidth]{figures/separated_extra_1024_1000_10.png}
    \caption{Separated with flow feature of the chosen packets, validation split=10\%, validation accuracy: 97\%} \label{fig:sep_extra}
    % \vspace{-0.4cm}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.45\textwidth]{figures/separated_extra_all_1024_1000_10.png}
    \caption{Separated with flow features of all packets, validation split=10\%, validation accuracy: 98\%} \label{fig:sep_all}
    % \vspace{-0.4cm}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.45\textwidth]{figures/separated_1024_1000_50.png}
    \caption{Separated, validation split=50\%, validation accuracy: 82\%} \label{fig:sep_50}
    % \vspace{-0.4cm}
\end{figure}

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.45\textwidth]{figures/separated_extra_1024_1000_50.png}
    \caption{Separated with flow feature of the chosen packets, validation split=50\%, validation accuracy: 83\%} \label{fig:sep_extra_50}
    % \vspace{-0.4cm}
\end{figure}

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.45\textwidth]{figures/separated_extra_all_1024_1000_50.png}
    \caption{Separated with flow features of all packets, validation split=50\%, validation accuracy: 86\%} \label{fig:sep_all_50}
    % \vspace{-0.4cm}
\end{figure}


==> sections/old_04-architecture.tex <==
\section{Intelligent Data Plane Neural Network} \label{sec:architecture}
In this part, we focus on the splitting problem of the DNNs to not only fit the model on a set of programmable switches but also to provide an efficient execution flow of the neural network. Further, we discuss the packet generation for the input and the generated intermediate data and address the DNN execution challenges in the switches.

\subsection{Mapper} \label{sec:mapper}
\cite{razavi2022distributed} suggested to partition DNNs layer by layer. We follow the same practice and assign each layer to a switch. Since there are layers without weights (MaxPooling, Flattening layers), we do not need to assign a switch to such layers. Therefore, we fit such layers with the previous layers with active weights (Convolutional and Dense layers) and perform the related operations of the earlier layers' operations. 

\begin{figure*}[!t]
    \centering
    \includegraphics[width=0.98\textwidth]{figures/mapping-cropped.pdf}
    % \vspace{-0.1cm}
    
    \caption{\namex{} Mapper} \label{fig:mapper_design}
    % \vspace{-0.4cm}
\end{figure*}

\noindent\textbf{Convolutional Layers}: We divide the number of filters by the available pipelines on a switch. The filter-splitting approach suits the switch architecture well since there is no communication between any two filters in the same convolutional layer, and filter computations can be done in parallel. For the model in Figure~\ref{fig:neuralnetwork}, each pipeline in the first switch receives 2 filters, while the second switch receives 4 filters per pipeline. In the inference phase, after the convolutional layers, there is a MaxPooling layer, which will be fit in the same switches as shown in Figure~\ref{fig:mapper_design}.

\noindent\textbf{Dense Layers}: We follow the same approach as in the convolutional layer, and instead of dividing the layer by the number of filters, we divide it by the number of dense neurons. Similar arguments apply here as there is no communication between two dense neurons in the same layer, and the dense neuron computations can be executed in parallel.

After mapping the layers to switches, we need to store the weights of the layers on the switches. We use register arrays (1D) for storing the weights. For storing the weight of the convolutional layers using the control plane, we can use $Filter \times Height \times Weight$ to map a number from $\mathbb{R}^3 \longrightarrow \mathbb{R}$. However, calculating the multiplications on the data plane is computationally expensive as multiplications are not natively supported on the programmable switches. Therefore, we use an available hash function on the data plane to create a unique index using similar identifiers ($Hash(Filter \times Height \times Weight)$). For storing the dense layer's weights, we add an index identifier to find the weights since they can be numbered from 0 to the total number of dense neurons on that specific layer.

So far, we have mapped a DNN with different layers (Convolutional, Dense, and MaxPooling) to a set of switches. Next, we need to generate the DNN computational flow using network packets.

\subsection{Packet Generator} \label{sec:generator}
When a packet arrives at a switch, we need to mimic the DNN flow execution using network packets. We first identify the next layer that the input/intermediate data should be sent and based on the layer type we follow different strategies.

\noindent\textbf{Convolutional Layers}: If the next layer type is a convolutional layer, we put the related data based on the kernel size of the convolutional layer to the packet header (including the necessary identifiers) and multicast the packet to all the next switch pipelines. The result of this approach is that when a packet arrives at a convolutional switch, it can perform all the necessary computations related to that exact packet header data, except the MaxPooling part (discussed in the Section~\ref{sec:executor}) as it requires multiple packet headers. When the data in the packet headers are processed, we get a final value for the current packet header that will be used to generate the next packet header based on the following switch type.

\noindent\textbf{Dense Layers}: If the next layer type is a dense layer, we multicast each data to all the next switch pipelines since each value is used by all the neurons of a dense layer. After all the computations regarding the current data are completed, the intermediate data is stored on the switch. After all the computations regarding a dense neuron are  finished, the finalized value is ready to be sent to the next switch pipelines based on the next switch type.

\subsection{P4 Executor} \label{sec:executor}
When a packet arrives in the initial switch, we capture the inter-arrival time and calculate the simple inter-arrival time features (min, max) up to the current packet. After that, we need to identify if the current packet is an inference point. Following NetBeacon~\cite{zhou2023efficient}, we check whether a packet is in the order of the power of 2 (1, 2, 4, ...) as it can be easily identified in a programmable switch. If a packet is an inference point, we start generating packets as described in the previous part. We use the following procedures (based on the layer type) to process the generated packets.

\noindent\textbf{Convolutional and MaxPooling Layers}: First, we create the hash of the indexes (filter number, height, and width) of the required weights. After the weights are fetched from registers, we perform dot productions for all the weights and the values. For the dot production, we can break down each multiplication operation into a series of bit-shifts. Specifically, we shift the input left by an amount determined by the corresponding bit in the 8-bit weight. These shifts are executed concurrently in a single processing stage, and the interim results are stored temporarily. Following this, a reduction step combines the interim results. Given that we employ 8-bit weights, this step necessitates three stages. To reduce the number of required stages, we store all possible dot products of 8-bit to 8-bit values and use a TCAM table to access the dot product of value|weight. This approach requires 1 stage instead of needing 3 stages for the dot product with the memory requirement of $2^{16}$ 8-bit values (65KB of memory). Next, we employ the ReLU activation function to process the dot product result. This involves examining the most significant bit (MSB), which serves as the sign bit, and substituting the value with 0 when it is set to 1.

To perform MaxPooling operations, we need to be sure that all the values regarding a MaxPooling window have arrived at the switch. To ensure that, we use a bitmap (using a table) of each value and flag its indexes when it arrives. Anytime a packet arrives, we check the bitmap of the value, and if all packets have arrived, we fetch the intermediate results of all the packets regarding the same MaxPooling window and find the maximum of the values within $log(size(MaxPooling window))$. After calculating the final value, we multicast it to the following switch pipelines.

\noindent\textbf{Dense Layers}: For the dense layer, finding the index of the dense neuron is relatively straightforward. When a packet arrives at a dense switch, we use a counter to find the weights and use the same dot product calculation as the one in the convolutional layers. After that, we aggregate the intermediate results until all variables from the previous layer are processed. After that, we perform a ReLU activation function to see if we want to activate the neuron. Finally, we multicast the result to the next switch pipelines.


\iffalse
\begin{table}[!t]
    \centering
    \footnotesize
    \caption{Notations}\label{table:notation}
    \begin{tabular}{ p{1.2cm}p{5.8cm}  }
        \toprule
        \textbf{Symbol} & \textbf{Description}\\
        \midrule
        $L$ & layers \\
        $I_w$ & input width \\
        $I_h$ & input height \\
        $A$ & number of ALUs per stage \\
        $S$ & number of stages \\
        $K_w$ & kernel width \\
        $K_h$ & kernel height \\
        $F$ & number of filters \\
        $M_w$ & maxpooling width \\
        $M_h$ & maxpooling height \\
        $P$ & number of pipelines \\
        $D_{in}$ & number of input for a dense layer \\
        $D_{out}$ & number of out for a dense layer \\
        \bottomrule
    \end{tabular}
    % \vspace{-0.4cm}
\end{table}

\subsubsection{Convolution}
Kernel by Kernel:
\begin{enumerate}
    \item We need $I_w - K_w + 1$ kernel boxes.
    \item Each box needs $k_w \times k_h$ dot products -> $ST_1 := \frac{k_w \times k_h}{A}$ stages.
    \item After the dot products, we need $ST_2 := log_2(k_w \times k_h)$ stages to aggregate the dot products.
    \item Total number of stages per filter without maxpooling: $ST_3 := \frac{(I_w - K_w + 1)}{\frac{ST_1 + ST_2}{A}}$.
    \item We need $M_w \times M_h$ values to perform a maxpooling window, which requires $ST_4 := log_2(M_w \times M_h)$ stages.
    \item We can perform $\frac{M_w \times M_h}{A}$ maxpooling operation per stage.
    \item Total number of stages per filter for maxpooling: $ST_5:= \frac{(I_w - K_w + 1)}{M_w} \times ST_4 \times \frac{M_w \times M_h}{A}$
    \item Total number of stages per filter: $ST_6 := ST_3 + ST_5$.
    \item Total number of stages per layer: $S_1 = F \times ST_6$.
    \item Number of needed pipelines: $P_1 = \frac{S_1}{S}$
    \item Number of needed switches for a convolutional layer: $N_d = \frac{P_1}{P}$
\end{enumerate}

\subsubsection{Dense}
Maximum operation per pipeline:
\begin{enumerate}
    \item We need $D_{in}\times D_{out}$ operation.
    \item Total number of pipelines: $P2 :=\frac{D_{in}\times D_{out}}{A \times S}$
    \item Total number of switches for a dense layer: $N_d = \frac{P2}{P}$
\end{enumerate}

Therefore, the total number of needed switches are:
\begin{equation}
    \sum_{c \in L_{convolution}}{N_c} + \sum_{l \in L_{dense}}{N_d}
\end{equation}


We first provide the computational time complexity of the layers of a model (in the current work, Conv2D, Dense, and MaxPooling2D) including the number of operations required per layer in a switch. Then we provide a DNN to a set of switches mapping approach with the consideration of the switch limitations (discussed in Section~\ref{sec:switch_limitation}).

To estimate the execution time a DL model, we need to estimate the execution time of its layers and the communication time since the total execution time of a model equals to the aggregation of the execution time of the independent layers and the layers' communication time. We assume that between switches communication cost is negligible compared to the model execution. Therefore, we calculate the number of needed operations of the layers as follows:

\noindent\textbf{Dense Layers}: The time complexity of a Dense layer is mainly determined by the matrix multiplication operation performed between the input tensor and the weight tensor, along with the addition of the bias term; therefore, We need $D_{in} \times D_{out}$ dot operations and the same amount of operations for aggregating the intermediate results of the dot products.

\subsection{Latency and Memory Properties}
To estimate the execution time a DL model, we need to estimate the execution time of its layers and the communication time since the total execution time of a model equals to the aggregation of the execution time of the independent layers and the layers' communication time. For the communication latency, we stick to the experiments to calculate the communication latency since it is highly dependent on the hardware and the used libraries. To have a more accurate execution time and memory requirement of the layers, we calculate the theoretical execution time and the memory usage of the layers as follows.

\noindent \textbf{Dense}: The memory usage of a Dense layer depends on the size of the input tensor ($n$), the number of units ($m$) in the layer, and the data type with a size ($s$) bytes used to represent the tensors. The memory usage can be estimated as follows:
\begin{enumerate}
    \item The input tensor requires a memory of $n \times s$ bytes.
    \item The weights tensor (which stores the connection weights) requires a memory of $n \times m \times s$ bytes.
    \item The bias tensor requires a memory of $n \times s$ bytes,  if applicable.
\end{enumerate}

Therefore, the total memory usage of a Dense layer can be approximated as:

\begin{equation}
    (n + n \times m + n) \times s
\end{equation}

The time complexity of a Dense layer in TensorFlow is mainly determined by the matrix multiplication operation performed between the input tensor and the weight tensor, along with the addition of the bias term.The time complexity can be expressed as:

\begin{equation}
    O(n \times m)
\end{equation}

This indicates that the time required to compute the output of a Dense layer scales linearly with the input size and the number of units.

\noindent \textbf{Conv2D}:
The memory usage of a Conv2D layer depends on the size of the input feature map ($h, w, c$), the number of filters in the layer ($f$), the filter size with the kernel of ($k_h, k_w$), and the data type with a size of ($s$) bytes used to represent the tensors. The memory usage can be estimated as follows:
\begin{enumerate}
    \item The input feature map requires a memory of $h \times w \times c \times s$ bytes.
    \item The kernel tensor (which stores the filter weights) requires a memory of $k_h \times k_w \times c \times f \times s$ bytes.
    \item The bias tensor requires a memory of $f \times s$ bytes, if applicable.
\end{enumerate}
Therefore, the total memory usage of a Conv2D layer can be approximated as:
\begin{equation}
    (h \times w \times c + k_h \times k_w \times c \times f + f ) \times s
\end{equation}

The time complexity of a Conv2D layer is mainly determined by the convolution operation performed on the input feature map using the filters.
The time complexity can be expressed as:
\begin{equation}
    O(h \times w \times k_h \times k_w \times f)
\end{equation}
This indicates that the time required to compute the output of a Conv2D layer scales with the product of the input feature map size, filter size, number of input channels, and number of filters.

\noindent \textbf{MaxPooling2D}:
The memory usage of a MaxPooling2D layer depends on the size of the input feature map ($h, w, c$), the pooling window size ($p_h$, $p_w$), and the data type with a size of $s$ bytes used to represent the tensors.
\begin{enumerate}
    \item The input feature map requires a memory of $h \times w \times c \times s$ bytes.
    \item The output feature map after max pooling has dimensions $\frac{h}{p_h} \times \frac{w}{p_w} \times c$ and requires a memory of the output dimension $\times s$ bytes.
\end{enumerate}
The memory usage can be estimated as follows:
\begin{equation}
    (h \times w + \frac{h}{p_h} \times \frac{w}{p_w}) \times c \times s
\end{equation}

The time complexity of a MaxPooling2D layer is mainly determined by the pooling operation performed on the input feature map ($h, w, c$), the pooling window size as $(p_h, p_w)$.
The time complexity can be expressed as:
\begin{equation}
    O(h \times w \times p_h \times p_w \times c)
\end{equation}

This indicates that the time required to compute the output of a MaxPooling2D layer scales with the product of the input feature map size, pooling window size, and number of channels.

Now that we have the layers' theoretical latency and memory properties, we can calculate the model execution time if we assume that the model has $L$ layers, where each layer $\in \{\text{Conv2D}$, $\text{Dense}$, or $\text{MaxPooling2D}\}$ and layers are executed one after the other:

\begin{equation}
    \sum_{i \in L} l_i
\end{equation}

where $l_i$ is the execution time of layer $i \in L$.

\subsection{Data Plane Approximation}
The number of mathematical operations differs from the theoretical time complexity order since the order excludes the order bellow the maximum power in the order resulting in reduction in the latency approximation. For instance, latency of a Dense layer is:
\begin{enumerate}
    \item $n \times m$ input to weight multiplication.
    \item $n \times m - n$ aggregation of the multiplications.
    \item $n$ bias aggregation.
\end{enumerate}
Therefore, the total number of mathematical operations for Dense layers is twice as the order:
\begin{equation}
    n \times m + n \times m - n + n = 2 \times n \times m
\end{equation}
Similar to the Dense layer mathematical operations, the number of mathematical operations for Conv2D can be calculated as:
\begin{equation}
    2 \times h \times w \times k_h \times k_w \times f
\end{equation}
and for the MaxPooling2D layers:
\begin{equation}
    2 \times h \times w \times p_h \times p_w \times c
\end{equation}

Furthermore, the memory access and mathematical operations data plane limitations (as explained in Section~\ref{sec:switch_limitation}) add more latency to the end-to-end execution approximation since a simple 8-bit to 8-bit multiplication with one memory access requires four steps~\cite{razavi2022distributed}. Therefore, all the above formulas will be four times more time consuming.
\fi

\iffalse
\noindent \textbf{Conv2D}: The computational time complexity of a 2D convolutional layer depends on the size of the input and output tensors, as well as the size of the convolutional kernel. If we assume the input tensor has dimensions $\text{in\_h}$, $\text{in\_w}$, $\text{c\_in})$ and the output tensor has dimensions $\text{out\_h}$, $\text{out\_w}$, $\text{c\_out})$. The convolutional kernel has dimensions $(\text{k\_h}$, $\text{k\_d}$, $\text{c\_in}$, $\text{c\_out})$.

The time complexity of a 2D convolutional layer can be estimated as follows:
\begin{enumerate}
    \item For each sample:
    \begin{enumerate}
        \item Slide the convolutional kernel over the input tensor, computing the dot product at each spatial location.
        \item Multiply each dot product by the corresponding kernel value and sum them.
        \item Add the bias term (if any).
        \item Apply any activation function (e.g., ReLU) to the resulting tensor.
    \end{enumerate}
    \item The sliding window operation has a time complexity of $O(\text{k\_h} \times \text{k\_d} \times \text{c\_in})$ per spatial location.
    \item The number of spatial locations is determined by the input and output dimensions, resulting in a time complexity of $O(\text{in\_h} \times \text{in\_w} \times \text{out\_h} \times \text{out\_w})$.
\end{enumerate}

Therefore, the overall time complexity of a 2D convolutional layer can be approximated as:
\begin{equation}
    O(\text{k\_h} \times \text{k\_d} \times \text{c\_in} \times \text{in\_h} \times \text{in\_w} \times \text{out\_h} \times \text{out\_w})
\end{equation}

\noindent \textbf{Dense}: The computational time complexity of a dense (fully connected) layer depends on the size of the input and output tensors. If we assume the input tensor has the dimension $\text{in\_s})$ and the output tensor has the dimension $\text{out\_s})$.

The time complexity of a dense layer can be estimated as follows:

\begin{enumerate}
    \item For each sample:
    \begin{enumerate}
        \item Perform a dot product between the input tensor of size $(\text{in\_s},)$ and the weight matrix of size $(\text{in\_s},$ $\text{out\_s})$.
        \item Add the bias term (if any).
        \item Apply any activation function (e.g., ReLU) to the resulting vector.
    \end{enumerate}
    \item The dot product operation between the input tensor and the weight matrix has a time complexity of $O(\text{in\_s})$.
\end{enumerate}

Therefore, the overall time complexity of a dense layer can be approximated as:
\begin{equation}
    O(\text{in\_s} \times \text{out\_s})
\end{equation}

\noindent \textbf{MaxPooling}: The computational time complexity of a MaxPooling layer depends on the size of the input and output tensors, as well as the size of the pooling window. If we assume the input tensor has dimensions $\text{in\_h}$, $\text{in\_w}$, $\text{channels})$ and the output tensor has dimensions $\text{out\_h}$, $\text{out\_w}$, $\text{channels})$. The pooling window has dimensions $(\text{pool\_h}$, $\text{pool\_w})$.

The time complexity of a MaxPooling layer can be estimated as follows:

\begin{enumerate}
    \item For each sample:
    \begin{enumerate}
        \item Slide the pooling window over the input tensor, selecting the maximum value within each window.
    \end{enumerate}
    \item The sliding window operation has a time complexity of $O(\text{pool\_h} \times \text{pool\_w})$ per spatial location.
    \item The number of spatial locations is determined by the input and output dimensions, resulting in a time complexity of $O(\text{in\_h} \times \text{in\_w} \times \text{out\_h} \times \text{out\_w})$.
\end{enumerate}

Therefore, the overall time complexity of a MaxPooling layer can be approximated as:

\begin{equation}
    O(\text{pool\_h} \times \text{pool\_w} \times \text{in\_h} \times \text{in\_w} \times \text{out\_h} \times \text{out\_w})
\end{equation}


Now that we have the layers' theoretical execution estimation times, we can calculate the model execution time (without the layers' communication time) if we assume that the model has $n$ layers, where each layer $\in \{\text{Conv2D}$, $\text{Dense}$, or $\text{MaxPooling2D}\}$ and layers are executed one after the other:

\begin{equation}
    \sum_{i \in n} l_i
\end{equation}

where $l_i$ is the execution time of layer $i \in n$.
\fi
